Training Deep Energy-Based Models with f-Divergence Minimization

Deep energy-based models (EBMs) are very flexible in distribution parametrization but computationally challenging because of the intractable partition function. They are typically trained via maximum likelihood, using contrastive divergence to approximate the gradient of the KL divergence between data and model distribution. While KL divergence has many desirable properties, other f-divergences have shown advantages in training implicit density generative models such as generative adversarial networks. In this paper, we propose a general variational framework termed f-EBM to train EBMs using any desired f-divergence. We introduce a corresponding optimization algorithm and prove its local convergence property with non-linear dynamical systems theory. Experimental results demonstrate the superiority of f-EBM over contrastive divergence, as well as the benefits of training EBMs using f-divergences other than KL.

==> background.tex <==
\section{Preliminaries}
\subsection{Energy-Based Generative Modeling}\label{sec:ebm-intro}
Suppose we are given a dataset consisting of \emph{i.i.d.} samples $\{\vx_i \}_{i=1}^N$ from an unknown data distribution $p(\vx)$, defined over a sample space $\gX \subset \mathbb{R}^m$. Our goal is to find a parametric approximation $q_\vtheta(\vx)$ to the data distribution, such that we can perform downstream inferences (\emph{e.g.}, density evaluation and  sampling). Specifically, we are interested in learning an (unnormalized) energy function $E_\vtheta(\vx)$ that defines the following normalized distribution:
\begin{align}
    q_\vtheta(\vx) = \exp(-E_\vtheta(\vx))/Z_{\vtheta},
\end{align}
where $Z_\vtheta = \int \exp(-E_\vtheta(\vx)) \mathrm{d} \vx$ 
%
is the normalization constant (also called the partition function). In this paper, unless otherwise stated, we will always use $p$ to denote the data distribution and $q_\vtheta$ to denote the model distribution. Moreover, we will assume $\exp(-E_\vtheta(\vx))$ is integrable over sample space $\gX$, \emph{i.e.}, $Z_\vtheta$ is finite. Because of the absence of the normalization requirement, energy-based distribution representation offers extreme modeling flexibility in the sense that we can use almost any model architecture that outputs a real number given an input as the energy function. 
%

While flexible, inference in EBMs is challenging because of the partition function, which is generally intractable to compute exactly. For example, it is non-trivial to sample from an EBM, which usually requires Markov Chain Monte Carlo (MCMC) \cite{robert2013monte} techniques.
As a gradient based MCMC method, Langevin dynamics \cite{neal2011mcmc,welling2011bayesian}
defines an efficient iterative sampling process, which asymptotically can produce samples from an energy-based distribution:
%
\begin{align}
    \Tilde{\vx}_t = \Tilde{\vx}_{t-1} - \frac{\epsilon}{2} \nabla_\vx E_\vtheta(\Tilde{\vx}_{t-1}) + \sqrt{\epsilon} \vz_t,
\end{align}
where $\vz_t \sim \mathcal{N}(0, I)$. The distribution of $\Tilde{\vx}_T$ converges to the model distribution $q_\vtheta(\vx) \propto \exp(- E_\vtheta(\vx))$ when $\epsilon \to 0$ and $T \to \infty$ under some regularity conditions \cite{welling2011bayesian}. 
%
Although few bounds on the mixing time are known, in practice researchers found that using a relatively small $\epsilon$ and finite $T$ suffices to produce good samples and
so far various scalable techniques have been developed for the purpose of sampling from an EBM efficiently. 
For example, 
%
\citet{du2019implicit} propose to use Langevin dynamics together with a sample replay buffer to reduce mixing time and improve sample diversity.
%

\subsection{The $f$-Divergence Family}\label{sec:f-div-family}
%
Let $P$ and $Q$ denote two probability distributions with density functions $p$ and $q$ with respect to a base measure $\mathrm{d} \vx$ on domain $\mathcal{X}$. Suppose $P$ is absolutely continuous with respect to $Q$, denoted as $P \ll Q$ (\emph{i.e.}, the Radon-Nikodym derivative $d P/d Q$ exists). For any strictly convex, lower-semicontinuous function $f: [0, +\infty) \to \mathbb{R}$ satisfying $f(1)=0$, the $f$-divergence between $P$ and $Q$ is defined as:
\begin{align}
    \DF(P\|Q) \defeq \int_\gX q(\vx) f\left(\frac{p(\vx)}{q(\vx)}\right) \mathrm{d} \vx
    = \mathbb{E}_{q(\vx)} \left[f\left(\frac{p(\vx)}{q(\vx)}\right)\right]. \nonumber
\end{align}
Many divergences are special cases obtained by choosing a suitable \emph{generator function} $f$. For example, $f(u) = u \log u$ and $f(u)=-\log u$ correspond to forward KL and reverse KL respectively (see Table 5 in \cite{nowozin2016f} for more examples). In the rest of this paper, we will consider the generator function $f$ to be strictly convex and continuously differentiable.

\begin{definition}[Fenchel Duality]
For any convex, lower-semicontinuous function $f: \gX \to \bb{R} \cup \{+ \infty\}$ defined over a Banach space $\gX$, the Fenchel conjugate function of $f$, $f^*$ 
%
is defined over the dual space $\gX^*$ as:
\begin{align}
    f^*(\vx^*) \defeq \sup_{\vx \in \gX} \langle \vx^*, \vx \rangle - f(\vx),
\end{align}
where $\langle \cdot, \cdot \rangle$ is the duality paring between $\gX$ and $\gX^*$. For a finite dimensional space $\bb{R}^d$, the dual space is also $\bb{R}^d$ and the duality paring is the usual vector inner product.
%
\end{definition}
 The function $f^*$ is also convex and lower-semicontinuous and more importantly, we have $f^{**} = f$, which means we can represent $f$ through its conjugate function as:
\begin{align}
    f(\vx) = \sup_{\vx^* \in {\gX}^*} \langle \vx^*, \vx \rangle - f^*(\vx^*).
\end{align}
Given samples from $P$ and $Q$, as well as the density of $Q$, it is generally intractable to directly estimate 
%
the $f$-divergences, because it requires to know the density ratio $p(\vx) / q(\vx)$. 
%
Based on Fenchel duality, \citet{nguyen2010estimating} proposed a general variational method to estimate $f$-divergences only using samples from $P$ and $Q$. 

\begin{definition}
Define the subdifferential $\partial f(\vx)$ of a convex function $f: \bb{R}^m \to \bb{R}$ at a point $\vx \in \bb{R}^m$ as the set:
$
    \partial f(\vx) \defeq \{\vz \in \bb{R}^m | f(\vy) \geq f(\vx) + \langle \vz, \vy - \vx \rangle, \forall \vy \in \bb{R}^m\}
$. 
When $f$ is differentiable at $\vx$, $\partial f(\vx) = \{\nabla_\vx f(\vx)\}$. 
%
\end{definition}

\begin{lemma}[\citet{nguyen2010estimating}]\label{lemma:f-bound}
Let $P$ and $Q$ be two probability measures over the Borel $\sigma$-algebra on domain $\gX$ with densities $p$, $q$ and $P \ll Q$.
For any class of functions $\gT$ mapping from $\gX$ to $\bb{R}$ such that the subdifferential $\partial f(p/q)$ contains an element of $\gT$, 
%
we have
%
\begin{equation}
    \DF(P \| Q) = \sup_{T \in \gT} \bb{E}_{p(\vx)} [T(\vx)] - \bb{E}_{q(\vx)}[f^*(T(\vx))],\label{eq:f-bound}
\end{equation}
where the supreme is attained at $T^*(\vx) = f'\left(\frac{p(\vx)}{q(\vx)}\right)$.
%
\end{lemma}

\subsection{Training Implicit Density Generative Models with Variational $f$-Divergence Minimization}\label{sec:variational-f-div}
For the purpose of training implicit density generative models (also known as generative neural samplers which are deterministic and differentiable mappings from noise space to sample space)
%
, \citet{nowozin2016f} proposed the following $f$-GAN objective to minimize the variational representation of $\DF(P\|Q_\vtheta)$ in Equation~(\ref{eq:f-bound}):
\begin{align}
    \min_\vtheta \max_\vomega \bb{E}_{p(\vx)}[T_\vomega(\vx)] - \bb{E}_{p(\vz)}[f^*(T_\vomega(G_\vtheta(\vz)))],\label{eq:f-gan}
\end{align}
where $p(\vz)$ is a fixed noise distribution (typically Gaussian distribution); $G_\vtheta: \gZ \to \gX$ is a direct differentiable mapping from noise space to sample space and $T_\vomega: \gX \to \bb{R}$ is the variational function. Note that the original GAN objective \cite{goodfellow2014generative} is also a special case with $f(u) = u \log u - (u+1) \log (u + 1)$.

\subsection{Tackling Intractable Partition Function with Contrastive Divergence} 
The predominant approach to training explicit density generative models is to minimize the KL divergence between the (empirical) data distribution and model distribution, which is a special member within the $f$-divergence family. Minimizing KL is equivalent to the following maximum likelihood estimation (MLE) objective:
\begin{align}
    \gL_{\mathrm{MLE}}(\vtheta; p) \defeq -\mathbb{E}_{p(\vx)}\left[\log q_\vtheta(\vx)\right].\label{eq:mle}
\end{align}
Because of the intractable partition function, we do not have access to the normalized density $q_\vtheta(\vx)$ and cannot directly optimize the MLE objective. Fortunately, we can use contrastive divergence \cite{hinton2002training} to estimate the gradients of Equation~(\ref{eq:mle}):
\begin{align}
    \nabla_\vtheta \gL_{\mathrm{MLE}}(\vtheta; p) &= \nabla_\vtheta \bb{E}_{p(\vx)}[E_\vtheta(\vx)] + \nabla_\vtheta \log Z_\vtheta \label{eq:contrastive-divergence}\\
    & =  \bb{E}_{p(\vx)}[\nabla_\vtheta E_\vtheta(\vx)] - \bb{E}_{q_\vtheta(\vx)}[\nabla_\vtheta E_\vtheta(\vx)].\nonumber
\end{align}
Intuitively this amounts to decreasing the energies of ``positive'' samples from $p$ and increasing the energies of ``negative samples'' from $q_\vtheta$.

As mentioned in Section~\ref{sec:ebm-intro}, MCMC techniques such as Langevin dynamics are needed in order to sample from $q_\vtheta$, which gives rise to the following surrogate gradient estimation:
\begin{align}
    \nabla_\vtheta \gL_{\mathrm{CD-}K}(\vtheta; p) = \bb{E}_{p(\vx)}[\nabla_\vtheta E_\vtheta(\vx)] - \bb{E}_{q_\vtheta^K(\vx)}[\nabla_\vtheta E_\vtheta(\vx)],\nonumber
\end{align}
where $q_\vtheta^K$ denotes the distribution after $K$ steps of MCMC transitions from an initial distribution (typically data distribution or uniform distribution), and Equation~(\ref{eq:contrastive-divergence}) corresponds to $\gL_{\mathrm{CD-}\infty}$. 

%
